Leveraging VLM-Based Pipelines to Annotate 3D Objects

Pretrained vision language models (VLMs) present an opportunity to caption unlabeled 3D objects at scale. The leading approach to summarize VLM descriptions from different views of an object (Luo et al., 2023) relies on a language model (GPT4) to produce the final output. This text-based aggregation is susceptible to hallucinations as it merges potentially contradictory descriptions. We propose an alternative algorithm to marginalize over factors such as the viewpoint that affect the VLM's response. Instead of merging text-only responses, we utilize the VLM's joint image-text likelihoods. We show our probabilistic aggregation is not only more reliable and efficient, but sets the SoTA on inferring object types with respect to human-verified labels. The aggregated annotations are also useful for conditional inference; they improve downstream predictions (e.g., of object material) when the object's type is specified as an auxiliary text-based input. Such auxiliary inputs allow ablating the contribution of visual reasoning over visionless reasoning in an unsupervised setting. With these supervised and unsupervised evaluations, we show how a VLM-based pipeline can be leveraged to produce reliable annotations for 764K objects from the Objaverse dataset.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> prior_work.tex <==



\subsection{Prior Work}

Before VLMs, one approach \cite{han2020shapecaptioner} to caption 3D shapes focused on detecting parts of an object across multiple views, then translating a sequence of view-aggregated part features into a caption. Another work \cite{koo2022partglot} showed that part segmentation was possible using human text-based annotations to discriminate between related shapes. 

Foreshadowing the possibilities for semantic annotation of 2D images, \cite{zareian2021open} explored novel object detection using sparse bounding box annotations but extensive image-caption data. With the advent of VLMs, more image processing and reasoning tasks came within reach: VISPROG \cite{Gupta_2023_CVPR} used in-context VLM learning to produce Python code to invoke off-the-shelf computer vision models and image processing APIs. ViperGPT \cite{suris2023vipergpt} also showed gains in reasoning spatially or at the level of object attributes by decomposing such queries into executable subroutines. Even closer to our work, \cite{zhu2023chatgpt} explored an interactive VQA approach using an LLM (ChatGPT) to ask questions about image contents, a VLM (BLIP-2) to answer them, and finally an LLM to produce a summary caption. \cite{gao2023physically} recently explored the inference of physical properties such as object material in images and collected a custom dataset to fine-tune VLMs.

Applying VLMs to 3D domains remains under-explored. \cite{ha2022semantic} propose using object category labels to extract relevancy maps from 2D VLMs. These can be turned into 3D occupancies, and then utilized for scene completion or object localization tasks. \cite{hong20233d} propose training 3D VLMs by projecting 3D feature maps into 2D and bootstrapping from a pretrained 2D VLM. The only method that contends with aggregating outputs from multiple VLM probes is ConceptGraphs \cite{gu2023conceptgraphs}, released when this work was submitted. Their focus is on building open-vocabulary scene graphs to help with navigation-related tasks in larger environments, which is different from our objective of generating object-centric, property-specific annotations.


